Packet Forwarding with a Locally Bursty Adversary

We consider packet forwarding in the adversarial queueing theory (AQT) model introduced by Borodin et al. We introduce a refinement of the AQT $(\rho, \sigma)$-bounded adversary, which we call a \emph{locally bursty adversary} (LBA) that parameterizes injection patterns jointly by edge utilization and packet origin. For constant ($O(1)$) parameters, the LBA model is strictly more permissive than the $(\rho, \sigma)$ model. For example, there are injection patterns in the LBA model with constant parameters that can only be realized as $(\rho, \sigma)$-bounded injection patterns with $\rho + \sigma = \Omega(n)$ (where $n$ is the network size). We show that the LBA model (unlike the $(\rho, \sigma)$ model) is closed under packet bundling and discretization operations. Thus, the LBA model allows one to reduce the study of general (uniform) capacity networks and inhomogenous packet sizes to unit capacity networks with homogeneous packets. On the algorithmic side, we focus on information gathering networks -- i.e., networks in which all packets share a common destination, and the union of packet routes forms a tree. We show that the Odd-Even Downhill (OED) forwarding protocol described independently by Dobrev et al.\ and Patt-Shamir and Rosenbaum achieves buffer space usage of $O(\log n)$ against all LBAs with constant parameters. OED is a local protocol, but we show that the upper bound is tight even when compared to centralized protocols. Our lower bound for the LBA model is in contrast to the $(\rho, \sigma)$-model, where centralized protocols can achieve worst-case buffer space usage $O(1)$ for $\rho, \sigma = O(1)$, while the $O(\log n)$ upper bound for OED is optimal only for local protocols.

==> lba.tex <==
\section{Locally Bursty Adversaries}

Here, we describe a more refined parametrization of adversarial injection patterns, and show how it arises naturally in several contexts. 

\begin{eg}
  \label{eg:local-burst}
  Let $G$ be the directed path of length $n+1$. Consider the adversary $A$ which in the first round injects a single packet into every buffer. Thereafter, only a single packet is injected into the first buffer, $1$. That is, 
  \[
  A = \set{(1, [i, n+1]) \sucht i \in [n]} \cup \set{(t, [n+1]) \sucht t \geq 2}
  \]
  It is natural to view the first injection as a single burst, while the asymptotic rate of the adversary is $1$, so that $A$ is $(1, n-1)$-bounded. Similarly, the injection pattern $A'$ that injects $n$ packets into buffer $1$ in round $1$, then $1$ packet per round thereafter is $(1, n-1)$-bounded. However, from the standpoint of buffer sizes, these injection patterns are very different. Simple greedy forwarding (i.e., every nonempty buffer forwards a packet each round) will deliver all packets from $A$ with buffers of size $1$, while $A'$ requires that $v_1$ has a buffer of size $n$.
\end{eg}

The example above illustrates that the $(\rho, \sigma)$-bounded adversarial model is not sufficiently refined to account for the space requirement to ``handle'' an injection pattern. We propose a more refined ``locally bursty'' adversarial model here. 

\begin{dfn}
  \label{dfn:local-burst}
  Let $A$ be an adversary, $\rho > 0$, and $\beta : V \to \N$. Then we say that $A$ is \dft{locally $(\rho, \beta)$-bounded} if for all finite intervals $T \subseteq \N$, subsets $S \subseteq V$ and $e \in E$, we have
  \[
  N_S^T(e) \leq \rho \abs{T} + \sum_{v \in S} \beta(v).
  \]
  That is, for every subset $S$ of nodes, the rate of injections into $S$ and crossing $e$ only ever exceeds $\rho$ by the sum of the $\beta(v)$ for $v \in S$. We denote the family of local $(\rho, \beta)$ bounded adversaries by $\calL(\rho, \beta)$.
\end{dfn}

\begin{eg}
  Consider the injection pattern $A$ from Example~\ref{eg:local-burst}. Viewing the initial injection as a local burst, we have $A \in \calL(1, \beta)$ for $\beta(i) = 1$ for all $i$. However, $A' \notin \calL(1, \beta)$. More generally, we have $\calL(\rho, \beta) \subset \calA(\rho, \sigma)$ for $\sigma = \sum_v \beta(v)$. The inclusion is strict unless exactly one $\beta(v)$ is positive, and as Example~\ref{eg:local-burst} shows, a $(\rho, \sigma)$-bounded injection pattern may be local $(\rho, \beta)$-bounded with $\beta(v) \ll \sigma$. 
\end{eg}

\begin{rem}
  \label{rem:general-burst}
  Definition~\ref{dfn:local-burst} can be generalized to include ``semi-local'' and global burstiness as follows. For every subset $R \subseteq V$, there is a parameter $\beta(R) \in \N$ which measures a maximum burst into the set $R$. For $\beta : 2^V \to \N$, an adversary $A$ is then $(\rho, \beta)$-bounded if for every $T \subseteq \N$ (finite), $S \subseteq V$, and edge $e$
  \[
  N_S^T(e) \leq \rho \abs{T} + \sum_{R : R \cap S \neq \varnothing} \beta(R).
  \]
  In the case where $\beta(R)$ is non-zero only when $R$ is a singleton set, we recover exactly Definition~\ref{dfn:local-burst}. If we set
  \[
  \beta(R) =
  \begin{cases}
    \sigma &\text{if } R = V\\
    0 &\text{otherwise},
  \end{cases}
  \]
  this generalized bound is equivalent to the $(\rho, \sigma)$-bounded adversary introduced by Cruz~[sic]. 
\end{rem}




\subsection{Meta-buffers}

In this section, we provide an alternate---perhaps more intuitive---description of locally $(\rho, \beta)$-bounded adversaries for fixed $\rho$ and $\beta$. The idea is to classify each packet injection as being either ``global'' or ``local.'' The interpretation is that each local injection into a buffer $e = (u, v)$ expends part of $e$'s ``burst budget,'' which cannot exceed $\beta(u)$ packets. On the other hand, the total number of global injections made during a time interval $T$ cannot exceed $\rho \abs{T}$---the average rate $\rho$ is never exceeded for global injections.

To formalize the idea above, we introduce the concept of a \dft{meta-buffer}. Each $e = (u, v) \in E$ has an associated meta-buffer, $\mu(e)$ which has a capacity of $\beta(v)$. We denote the set of meta-buffers by $M$. To distinguish $e$ from its associated meta-buffer, we refer to $e$ as the \dft{physical buffer}. Initially, at time $t = 0$, each $\mu(e)$ is initialized to contain exactly $\beta(e)$ packets. The adversary can inject packets into the network via local or global injections: a \dft{local injection} of $k$ packets into buffer $v(e)$ has the effect of removing $k$ packets from $\mu(e)$ and adding them to $e$. A \dft{global injection} into a buffer increments the buffer without decrementing the associated meta-buffer. Global injections may be made into either physical buffers or meta-buffers; injections into a meta-buffer $\mu(e)$ have the effect of ``replenishing'' the burst budget of the physical buffer $e$. When the pattern of global injections obeys a (global) $(\rho, 0)$-bound and the size of each meta-buffer $\mu(e)$ never exceeds $\beta(e)$, we refer to an execution of the injection process above as a \dft{$(\rho, \beta)$-bounded meta-buffer process}, and we say that the injection pattern is \dft{realized} by such a process.

We emphasize that an (online) forwarding protocol sees only the physical injection pattern. It cannot distinguish between global and local injections, and it does not see the state of the meta-buffers at any given time. %In Section~\ref{sec:buffer-size-}, we will show that from the perspective of buffer size minimization, knowing the state of the meta-buffers is essentially equivalent to knowing the entire future of an execution.

The following proposition shows that every local $(\rho, \beta)$-bounded adversary can be viewed as an execution of a $(\rho, \beta)$-bounded meta-buffer process, and vice versa. Thus, when considering any local $(\rho, \beta)$-bounded injection pattern, we may refer to the state of the meta-buffers of the execution.

\begin{prop}
  \label{prop:local-meta-buffer}
  Suppose $A$ is an injection pattern, $\rho > 0$, and $\beta : V \to \N$. Then $A \in \calL(\rho, \beta)$ if and only if $A$ is realized by a $(\rho, \beta)$-bounded meta-buffer process.
\end{prop}

Before proving the proposition, we introduce some notation.

\begin{dfn}
  \label{dfn:active-saturated}
  Suppose $P$ is a $(\rho, \beta)$-bounded meta-buffer process, and $t \in \N$. Then we say that a meta-buffer $\mu(v)$ is \dft{active} after time $t$ if $\mu(v)$ receives a global injection at some time $s > t$. We say that $\mu(v)$ is \dft{saturated} at time $t$ if $\abs{\mu^t(v)} = \beta(v)$, and \dft{unsaturated} otherwise. We denote the sets of active and unsaturated buffers at time $t$ by $\A(t)$ and $\U(t)$, respectively:
  \begin{align*}
    \A(t) &= \set{v \in V \sucht \mu(v) \text{ is active at some time } s > t},\\
    \U(t) &= \set{v \in V \sucht \abs{\mu^t(v)} < \beta(v)}.
  \end{align*}
\end{dfn}

\begin{proof}
  We first show the $\Leftarrow$ direction. Suppose $A$ is realized by a $(\rho, \beta)$-bounded meta-buffer process. Fix $r, t \in \N$ with $r \leq t$, and $S \subseteq [n]$. We must show that the number of packets $N(V_S, r, t)$ injected into $V_S$ during the time interval $[r, t]$ is at most $\rho (t - r + 1) + \sum_{i \in S} \beta_i$. To this end, let $\Gamma_S = (\gamma^r, \gamma^{r+1}, \ldots, \gamma^t)$ denote the pattern of \emph{global} injections made into $V_S$ and $M_S$, where
  \[
  V_S = \set{v_i \sucht i \in S}, \quad\text{and}\quad M_S = \set{\mu_i \sucht i \in S}.
  \]
  Then by the definition of a $(\rho, \beta)$-bounded meta-buffer process, we have
  \[
  \abs{\gamma^r} + \abs{\gamma^{r+1}} + \cdots + \abs{\gamma^t} \leq \rho(t - r + 1),
  \]
  because the global injections form a (global) $(\rho, 0)$-bounded injection pattern. During the interval $[r, t]$, the number of physical injections into $V_S$ can only exceed the number of global injections into $V_S \cup M_S$ by the size of the meta-buffers in $M_S$ at time $r$, so we obtain
  \begin{align*}
    N(V_S, r, t) \leq \rho(t - r + 1) + \sum_{i \in S} \abs{\mu_i(r)} \leq \rho (t - r + 1) + \sum_{i \in S} \beta_i,
  \end{align*}
  which gives the desired result.

  Now suppose $A \in \calL(\rho, \beta)$, and assume towards a contradiction that $A$ is not realized by any $(\rho, \beta)$-bounded meta-buffer process. Therefore, there exists some minimal round $t^*$ such that the subsequence $A' = (A^1, A^2, \ldots, A^{t^* - 1})$ is realizable, but $A'' = (A^1, \ldots, A^{t^*})$ is not. In particular, for any $(\rho, \beta)$-bounded meta-buffer process $P$ realizing $A'$, any extension of $P$ to round $t^*$ that ``realizes'' $A''$ must contain a meta-buffer $\mu_i$ with negative load---i.e., some meta-buffer must have injected more packets than it contained in round $t^*$. For any extension $P$ of any process realizing $A'$, we define the \dft{deficiency} of $P$, denoted $\defic(P)$ to be the number of packets injected by $A''$ in round $t^*$ that cannot be fulfilled by $P$:
  \[
  \defic(P) = \sum_{i \in [n]} \max\set{a_i(t^*) - \mu_i(t^* - 1) - \gamma_i(t^*), 0}.
  \]
  Fix some $P$ that minimizes $\defic(P)$ (which is positive by assumption). Let $D \subseteq [n]$ denote the set of \dft{deficient} meta-buffers for $P$:
  \[
  D = \set{i \in [n] \sucht a_i(t^*) - \mu_i(t^* - 1) - \gamma_i(t^*) \leq 0}.
  \]
  That is, $D$ is the set of meta-buffers whose loads would be non-positive after fulfilling the injection pattern specified by $A$ in round $t^*$. Similarly we define $S \subseteq D$ to be the set of \dft{strictly deficient} buffers:
  \[
  S = \set{i \in [n] \sucht a_i(t^*) - \mu_i(t^* - 1) - \gamma_i(t^*) < 0}.
  \]
  The idea of the proof is to find a set $D'$ with $S \subseteq D' \subseteq D$, such that
  \begin{enumerate}
  \item every meta-buffer $i \in D'$ is saturated at time $s$,
  \item $D'$ contains all nodes active after time $s$ (cf.\ Definition~\ref{dfn:active-saturated}), and
  \item $\rho(t^* - s)$ global injections were made into $D'$ during the intreval $[s + 1, t^*]$.
  \end{enumerate}
  Once we have shown that there exist $D'$ and $s$ satisfying conditions 1--3, we will show that these conditions contradict the assumption that $A \in \calL(\rho, \beta)$.

  %% Let $s$ be the maximal time $s < t^*$ such that every $\mu_i \in S$ is saturated (i.e., $\mu_i(s) = \beta_i$ for all $\mu_i \in S$). Note that $s$ is well-defined because every $\mu_i \in S$ is saturated at time $s = 0$. 
  \begin{description}
  \item[Claim 1.] There exists $s < t^*$ such that $A(s) \subseteq D$, and for all $i \in \A(s) \cup S$ we have $\mu_i(s) = \beta_i$.
  \item[Proof of Claim 1.] If $\A(0) \subseteq D$, then we are done as $\mu_i(0) = \beta_i$ for all $i$. Otherwise, set $t_0 = \max\set{t \sucht A(t) \not\subseteq D} + 1$---i.e., $t_0$ is the latest time at which some global injection into a buffer outside of $D$ occurs. Let $j \notin D$ be a meta-buffer which receives a global injection at time $t_0$.  The idea is to show that we can either ``forward'' this injection to a buffer $i \in S$ thereby decreasing the deficiency of $P$, or find a time $s > t_0$ satsifying the conditions of the claim.

    First, observe that for all $t \geq t_0$, we have $\mu_j(t) > 0$. This is because $\mu_j(t^*) > 0$, and by the maximality of $t_0$, $\mu_j$ did not receive any injections during the interval $[r + 1, t^*]$. Therefore, we can take a single packet injected into $\mu_j$ in round $t_0$ and instead inject it into another meta-buffer $\mu_i$ without violating the positivity of $\mu_j$. Note that at time $s = t_0$, either Claim~1 holds, or one of the following conditions holds:
    \begin{enumerate}[label=\Alph*.]
    \item there exists $i \in S$ such that $\mu_i(t) < \beta_i$ for all $t \in [s, t^*]$;
    \item there exists $i \in \A(s) \cup S$ such that $\mu_i(t) < \beta_i$.
    \end{enumerate}
    If condition~A holds, then by injecting a packet into $\mu_i$ instead of $\mu_j$, we can decrease the deficiency of $P$, thus contradicting its minimality. Therefore, assume condition~A is not satisfied, and condition~$B$ holds. Choose $i_0 \in (\A(t_0) \cup S) \cap U(t_0)$ arbitrarily, and define the meta-buffer injection process $P_0$ to be identical to $P$, except that one global injection into $\mu_j$ at time $t_0$ is made instead to $\mu_{i_0}$.\footnote{$P_0$ will fail to be $(\rho, \beta)$-bounded if there was some $t > t_0$ such that $\mu_{i_0}(t) = \beta_j$, however $P_0$ is $(\rho, \beta)$-bounded up to time $t_0$}

    We now define a sequence of pairs $(t_0, i_0), (t_1, i_1), \ldots$ with $t_0 < t_1 < \cdots$, and $i_k \in \A(t_k)$ for all $k$, together with meta-buffer processes $P_0, P_1, \ldots$ as follows. Given $t_{k-1}$ and $i_{k-1}$, let $t_k > t_{k-1}$ be the minimum of $\max\set{t > t_{k-1} \sucht i_{k-1} \in \A(t)}$ and $\min\set{t > t_{k-1} \sucht i_{k-1} \in \U(t)}$. That is, $t_k$ is either the last time that $i_{k-1}$ receives and injection, or the next time that $i_{k-1}$ is saturated. In either case, $i_{k-1}$ receives an injection at time $t_k$. If the conclusion of Claim~1 holds for $s = t_k$, then we are done. Otherwise, condition~A or~B above holds. If condition~A holds, let $i_k \in S$ be a meta-buffer satisfying condition~A; otherwise take $i_k \in (\A(t_k) \cup S) \cap \U(t_k)$ arbitrarily. Define the injection process $P_k$ to be identical to $P_{k-1}$ except that at time $t_k$, one injection made to $\mu_{i_{k-1}}$ is instead made to $i_k$.

    Obeserve that for each $k$, $P_k$ is $(\rho, \beta)$-bounded at least up to time $t_k$. In the case where condition~A is satisfied at time $t_k$, the new injection pattern $P_k$ is $(\rho, \beta)$-bounded for the entire interval $[0, t^*]$. Further, the deficit of $P_k$ is strictly smaller than the deficit of $P$, thereby contradicting the minimality of the deficit of $P$. Therefore, condition~A must never have occured in our construction of the sequence $(t_0, i_0), (t_1, i_1), \ldots$. If no time $t$ satisfying the condition of the claim is ever encountered, then we must have $t_0 < t_1 < \cdots < t_k = t^* - 1$. However, the fact that condition~A does not occur at $t_k$ implies that for all $i \in S$, $\mu_i(t_k) = \beta_i$. Therefore, $A$ injects strictly more than $\rho + \sum_{i \in \A(t_k) \cup S} \beta_i$ packets into buffers in $\A(t_k) \cup S$ during round $t^*$, contradicting the $(\rho, \beta)$-bound for $A$. Therefore there is some $s < t^*$ satisfying the conclusion of Claim~1.
  \end{description}

  Now let $s$ be the maximal time $s < t^*$ satisfying the conclusion of Claim~1, and let $D'$ be the corresponding subset of $D$.

  \begin{description}
  \item[Claim 2.] During the interval $[s + 1, t^*]$, $P$ makes $\rho(t^* - s)$ global injections into $D'$.
  \item[Proof of Claim 2.] Suppose for the sake of contradiction that at some time $t_0 \in [s+1, t^*]$ fewer than $\rho$ global injections are made. By the maximality of $s$, there exists some $i_0 \in \A(t_0) \cup S$ satisfying $\mu_{i_0}(t_0) < \beta_{i_0}$. Thus, an extra packet can be injected into $\mu_{i_0}$ at time $t_0$ without violating the $(\rho, \beta)$-bound up to time $t_0$. By constructing a sequence $(t_0, i_0), (t_1, i_1), \ldots$ as in the proof of Claim~1, we either encounter some $t_k > s$ also satisfying the conclusion of Claim~1, or we can construct a $(\rho, \beta)$-bounded meta-buffer process $P_k$ with smaller deficit than $P$. In the former case, we violate the maximality of $s$, and in the latter the minimality of the deficit of $P$. Thus, Claim~2 follows.
  \end{description}
  
  In order to finish the proof of the proposition, note that by Claims~1 and~2, there exist a time $s$ and subset $D'$ satisfying $S \subseteq D' \subseteq D$ such that for all $i \in D'$, $\mu_i(s) = \beta_i$ and $\rho(t^* - s)$ global injections were made into buffers $\mu_i$ for $i \in D'$ during the interval $[s+1, t^*]$. Therefore, the number of packets injected by $A$ into the physical buffers $v_i$ for $i \in D'$ was strictly greater than $\rho(t^* - s) + \sum_{i \in D'} \beta_i$, which contradicts the $(\rho, \beta)$-bound for $A$.
\end{proof}

\subsection{Rounding and Bundling}

The majority of the literature on adversarial queueing theory focuses on the case where all edges have unit capacity and $\rho \leq 1$. One reason for this is that it is harder to reason about larger capacities. Generalizing results for $\rho \leq 1$ to arbitrary $\rho$ is often a subtle problem. One of our motivations for introducing the local burst model is that it characterizes injection processes that arise from a ``round-and-bundle'' strategy for dealing with general edge capacities and injection rates $\rho > 1$.

The idea of the ``round-and-bundle'' strategy for $\rho > 1$ is to bundle $\rho$ packets together into ``jumbo packets'' and deal only with complete bundles. If a physical buffer $v$ contains $L(v)$ packets, then we treat these packets as $\floor{L(v) / \rho}$ jumbo packets, and ignore the remainder. Then any unit-capacity algorithm can be applied to forward jumbo packets. The problem with this approach is that if $\rho$ is large, then the unit-capacity algorithm may see large bursts of jumbo packets. For example, consider the case where $\rho = n$, and the adversary injects a single packet into each buffer during the first $n$ rounds. In the first $n - 1$ rounds, all buffers have fewer than $n$ packets, so no jumbo packets appear in the network. But at time $n$, the algorithm witnesses a burst of size $n$ in the entire network.

More generally, for a global $(\rho, \sigma)$-bounded adversary, the empirical injection pattern of jumbo packets under the round-and-bundle strategy is $(1, \sigma / \rho + \rho)$-bounded. Since upper bounds for buffer sizes tend to be of the form $f(\rho, n) + \sigma$, the corresponding bounds under the round-and-bundle strategy will be $\Omega(f(1, n), \sigma / \rho + \rho)$, which may be dominated by the additive $\rho$. However, the bursts of jumbo packet injections are not arbitrary (as are bursts allowed in the global $(\rho, \sigma)$-bounded adversarial model): each buffer can only see bursts of a single jumbo packet. The resulting injection pattern is a locally bursty adversary where the local burst size is only 1. Thus, if a unit-capacity algorithm performs well against locally bursty adversaries, its performance will carry over to arbitrary $\rho$ using the round-and-bundle strategy. Moreover, this strategy can be used to deal with continuously divisible packets and aribtrary heterogeneous packet sizes in a unified manner. Here, we formalize these ideas and prove some basic results.

\begin{dfn}
  Let $A$ be an injection pattern an $\rho \in \N$, $\rho \geq 2$. For $v \in V$ and $t \in \N$, let $A(v, t) = \sum_{s \leq t} a_v(t)$ denote the total number of packets injected into $v$ up to time $t$. Then we define the \dft{$\rho$-bundled} injection pattern $A_\rho$ is defined by $A_\rho(v, t) = \floor{A(v, t) / \rho}$ for all $t \in \N$.
\end{dfn}

\begin{prop}
  \label{prop:bundling}
  Suppose $A$ is a generalized $(\rho, \beta)$-bounded adversary (as in Remark~\ref{rem:general-burst}), and $A_\rho$ the corresponding $\rho$-bundled injection pattern. Then $A_\rho$ is $(1, \beta')$-bounded where for every subset $T \subseteq [n]$
  \[
  \beta'_T =
  \begin{cases}
    \frac{1}{\rho} \beta_T + 1 &\text{if } \abs{T} = 1\\ \frac{1}{\rho} \beta_T & \text{otherwise}.
  \end{cases}
  \]
\end{prop}
\begin{proof}
  Let $B = A_\rho$ so that $b_i(t)$ is the number of packets injected by $B$ into $i$ at time $t$. Fix any subset $S \subseteq [n]$ and times $r, t \in \N$ with $r \leq t$. We compute
  \begin{align*}
    \sum_{s = r}^t \sum_{i \in S} b_i(t) &= \sum_{i \in S} \paren{\floor{\sum_{s = 0}^t a_i(t) / \rho} - \floor{\sum_{s = 0}^{r-1} a_i(t) / \rho}}\\ &\leq \sum_{i \in S} \paren{\floor{\sum_{s = r}^t a_i(t) / \rho} + 1}\\ &\leq \abs{S} + \frac{1}{\rho}\sum_{i \in S} \sum_{s = r}^t a_i(t)\\ &= \abs{S} + \frac{1}{\rho} \paren{\rho(t - r + 1) + \sum_{T : S \cap T \neq \varnothing} \beta_T}\\ &\leq \abs{S} + t - r + 1 + \sum_{T : S \cap T \neq \varnothing} \frac{1}{\rho} \beta_T\\ &= t - r + 1 + \sum_{T : S \cap T \neq \varnothing} \beta'_T,
  \end{align*}
  which gives the desired result.
\end{proof}

Proposition~\ref{prop:bundling} gives a simple and unified means of generalizing algorithms and upper bounds for $\rho = 1$ adversaries to general $\rho > 1$ adversaries. We now describe two related packet injection models. In the first, packets are treated as continuous entities that can be divided arbitrarily. In the second model, packets are discrete and indivisible, but have an arbitrary associated weight which corresponds to the packet's size.

\subsubsection{Continuous Packet Injections}

\subsubsection{Heterogeneous Packet Injections}

